Automata for Hyperlanguages

Hyperproperties lift conventional trace properties from a set of execution traces to a set of sets of execution traces. Hyperproperties have been shown to be a powerful formalism for expressing and reasoning about information-flow security policies and important properties of cyber-physical systems such as sensitivity and robustness, as well as consistency conditions in distributed computing such as linearizability. Although there is an extensive body of work on automata-based representation of trace properties, we currently lack such characterization for hyperproperties. We introduce hyperautomata for em hyperlanguages, which are languages over sets of words. Essentially, hyperautomata allow running multiple quantified words over an automaton. We propose a specific type of hyperautomata called nondeterministic finite hyperautomata (NFH), which accept regular hyperlanguages. We demonstrate the ability of regular hyperlanguages to express hyperproperties for finite traces. We then explore the fundamental properties of NFH and show their closure under the Boolean operations. We show that while nonemptiness is undecidable in general, it is decidable for several fragments of NFH. We further show the decidability of the membership problem for finite sets and regular languages for NFH, as well as the containment problem for several fragments of NFH. Finally, we introduce learning algorithms based on Angluin's L-star algorithm for the fragments NFH in which the quantification is either strictly universal or strictly existential.

==> NBH.tex <==







We now lift the notion of hyperautomata to infinite words. 
A {\em hyper-infinite word} over $\Sigma$ is a set of infinite words over $\Sigma$. 
As before, an automaton $\A$ for a hyperlanguage $\cal L$ consists of an underlying automaton which runs on the tuples of words that are assigned to the word variables of $\A$. In the case of hyper-infinite words, the underlying automaton runs on tuples of infinite words. We consider a B{\"u}chi acceptance condition for the underlying automata. 

\begin{definition}
A {\em nondeterministic B{\"u}chi hyper-word automaton (NBH)} is a tuple $\A = 
\tuple{\Sigma, X=\{x_1,\ldots x_k\}, Q, Q_0, \delta, F, \alpha}$, where all 
elements are as in NFH and acceptance condition defined by the underlying NBW 
of $\A$ is $\hat{\A} = \tuple{\Sigma^k,Q,Q_0,\delta,F}$.

\end{definition}

In particular, consider a hyper-infinite word $S$ and an 
assignment $v:X\rightarrow S$. Then $\hat\A$ accepts $\zip(v)$ iff the run of 
$\hat\A$ on $\zip(v)$ visits some state in $F$ infinitely often. 
The definition of $\models$, acceptance, and $\lang{A}$ are all as in NFH.
As with NFH, we consider the different fragments of NBH$_\forall$, NBH$_\exists$, NBH$_{\forall\exists}$ and NBH$_{\exists\forall}$.


\subsection{Properties of NBH}

Since NBWs are closed under the Boolean operations, and their nonemptiness and inclusion problems are decidable (and are NL-complete and PSPACE-complete, respectively), the results of Section~\ref{sec:nfh_properties} can all be lifted to the case of hyper-infinite words. 
To summarize, we have the following. 

\begin{theorem}
\begin{itemize}
    \item NBH are closed under the Boolean operations.
    \item The nonemptiness problem for NBH$_\exists$ is NL-complete.
    \item The nonemptiness problem for NBH$_{\exists\forall}$ is decidable in EXPSPACE.
    \item The nonemptiness problem for NFH$_{\forall\exists}$ is undecidable.
    \item The $\omega$-regular membership problem for NBH is decidable.\todo{this is just a bit trickier, since we need to be more careful with the accepting states}
\end{itemize}
\end{theorem}



==> NBHtoHLTL.tex <==
\section{HyperLTL to HyperABA}

\todo{BB: I think we should clearly define HyperLTL and ABA if we want to keep 
this section. I also think this construction appears in 
https://www.react.uni-saarland.de/publications/FRS15.pdf.}\todo{Sarai: I agree about the definitions. About this construction, it's a little different since there the construction is directly for the purpose of model checking and has the system "built in", so there is no quantification of the automaton, it's a standard word automaton. But indeed the idea is similar. Perhaps we should minimize this section and mention that an extension to infinite words allows a direct translation of hyperltl to hyperautomata}

Let $AP$ be a set of atomic propositions, and let $\g = \quant_1 x_1 \ldots \quant_k x_k \f$ be a hyper-LTL formula. 
We construct a hyper-ABA $\A_\g$ over $(2^{AP})^k$ that accepts a hyperword $S$ iff $S\models\f$. Our construction is directly based on Vardi and Wolper's construction for LTL. 
The set of states $S$ is $sub(\f)$, the set of sub-formulas of $\f$, the initial state is $\f$, the set of accepting states are all subformulas of the type $\neg \f_1\until\f_2$.
To define the transition relation $\delta$, 
we first define the {\em dual} formula $\overline{\alpha}$ for a formula $\alpha$, as follows. Let $\alpha_1,\alpha_2$ be formulas over $S$. 
\begin{itemize}
    \item $\overline{\true} = \false$ and $\overline{\false}=\true$.
    \item $\overline{\alpha} = \neg\overline{\alpha}$, for $\alpha\in S$.
    \item $\overline{\alpha_1\wedge\alpha_2} = \overline{\alpha_1}\vee\overline{\alpha_2}$.
    \item $\overline{\alpha_1\vee \alpha_2} = \overline{\alpha_1}\wedge\overline{\alpha_2}$.
    \item

\end{itemize}

The transition relation $\delta$ is as follows. 
\begin{itemize}
\item $\delta(a_{x_i},\sigma) = \true$ if $a\in\sigma[i]$, and $\false$ otherwise. 
\item $\delta(\nextt \f_1, \sigma) =  \f_1$.
\item $\delta(\f_1\vee \f_2,\sigma) = \delta(\f_1,\sigma)\vee \delta(\f_2,\sigma)$.
\item $\delta(\neg \f_1) = \overline{\delta(\f_1)}$.
\item $\delta(\f_1 \until \f_2, \sigma) = \delta(\f_2,\sigma)\vee (\delta(\f_1,\sigma) \wedge (\f_1\until\f_2))$. 
\end{itemize}

Finally, the quantification condition of $\A_\g$ is $\quant_1 x_1 \ldots \quant_k x_k$. 

==> canonical_forms_full.tex <==

\subsection{Canonical Forms for Alternation-free Fragment}

Throughout this section, we discuss NFH over an alphabet $\Sigma$ with a set of 
variables $X = \{x_1,x_2,\ldots x_k\}$.

\subsubsection{A Canonical Form for $\nfhf$}

We begin with a canonical form for $\nfhf$. Let $\A$ be an $\nfhf$. 
We say that an $\nfhf$ $\A'$ is {\em sequence complete} if for every word $w$, it holds that $\hat \A'$ accepts $w$ iff it accepts every sequence of $w$. 

\begin{lemma}
\label{lem:langeq}
Let $\A'$ be a sequence complete $\nfhf$ over $\Sigma$ and $X$, such that 
$\hat\A'$ accepts $w$ iff $\hat\A$ accepts every sequence of $w$. 
Then $\lang{\A} =\lang{\A'}$.
\end{lemma}


\begin{lemma}
\label{lem:eqseq}
Every $\nfhf$ $\A$ has an equivalent sequence-complete $\nfhf$ $\A'$ over the 
same set of variables. 
\end{lemma}

\begin{lemma}
\label{lem:seqcomp}
Let $\A_1$ and $\A_2$ be two sequence-complete $\nfhf$ over the same set of 
variables $X$.
Then $\lang{\A_1}=\lang{\A_2}$ iff  $\lang{\hat\A_1} = \lang{\hat \A_2}$.
\end{lemma}

Every NFA has an equivalent DFA, and DFAs have a canonical form, which is a 
minimal DFA. We use this property to define a canonical form for $\nfhf$ as 
minimal deterministic sequence-complete $\nfhf$ with a minimal number of 
variables. 


\subsubsection{A Canonical Form for $\nfhe$}

We say that an $\nfhf$ $\A'$ is {\em permutation complete} if for every word 
$w$, it holds that $\hat \A'$ accepts $w$ iff it accepts every permutation of 
$w$. 

\begin{lemma}
\label{lem:premcomp}
Let $\A$ be an $\nfhe$.
Let $\A'$ be a permutation-complete $\nfhe$ over $\Sigma$ and $X$ with the following property: for every word $w$, the underlying NFA $\hat\A$ accepts a word $w$ iff $\hat\A'$ accepts all permutations of $w$. %Notice that this is the dual property of the one listed for $\nfhf$.
Then $\lang{\A} =\lang{\A'}$.
\end{lemma}

\begin{lemma}
\label{lem:eqpermcomp}
Every $\nfhe$ has an equivalent permutation-complete $\nfhe$ over the same set 
of variables. 
\end{lemma}

\begin{lemma}
\label{lem:permcompsame}
Let $\A_1$ and $\A_2$ be two permutation-complete $\nfhe$ over the same set of 
variables $X$.
Then $\lang{\A_1}=\lang{\A_2}$ iff  $\lang{\hat\A_1} = \lang{\hat \A_2}$.
\end{lemma}

We define a canonical form for $\nfhe$ as a minimal deterministic 
permutation-complete $\nfhe$ with a minimal number of variables.




\stam{

\subsubsection{A canonical form for $\nfhef$}

The canonical form for $\nfhef$ is a combination of the canonical forms for 
$\nfhf$ and $\nfhe$.

We denote an $\nfhef$ $\A$ with a quantification condition $\alpha = \exists 
x_1\ldots \exists x_t\forall k_{t+1}\ldots \forall x_k$ as a $(k,t)-\nfhef$. 

We say that a $(k,t)-\nfhef$ $\A$ is {\em permutation-sequence complete} if 
$\A$ accepts a word $w$ iff $\A$ accepts every sequence $w'$ of $w$ in which 
$(w'[1],\ldots w'[t])$ is a permutation of $(w[1],\ldots w[t])$. 

\begin{lemma}\label{lem:nfhef1}
Let $\A$ be a $(k,t)-\nfhef$. 
Let $\A'$ be a $(k-t)-\nfhef$, with the following property.
$w'\in\lang{\A'}$ iff $w'$ is a sequence of a word $w\in\lang{\hat\A}$ such that
\begin{enumerate}
\item
$(w'[1],\ldots w'[t])$ is a permutation of $(w[1],\ldots w[t])$. 
\item
$w_\zeta\in\lang{\hat\A}$ for every sequence $\zeta$ such that $\zeta = (1,2,\ldots t,i_{t+1},\ldots i_k)$. That is, $\hat\A$ accepts all sequences of $w$ that agree with $w$ on its first $t$ words. 
\end{enumerate}
Then $\lang{\A} = \lang{A'}$.
 \end{lemma}
\begin{proof}
For the first direction, let $S\in\lang{A}$. According to the semantics of the quantifiers, there exist $w_1,\ldots w_t\in S$, such that for every $w_{t+1},\ldots w_{k}$, it holds that $\hat\A$ accepts $\zip(w_1,\ldots w_k)$.
Then, by the semantics of the $\forall$ quantifier, $\hat\A$ accepts all words of the form $\zip(w_1,w_2,\ldots w_t,w'_{t+1},\ldots w'_k)$, where $w'_{t+1},\ldots w'_k$ are taken from $\{w_1,\ldots w_k\}$. Then, by the conditions described above, we have that $\hat\A'$ accepts $\zip(w_1,\ldots w_k)$, and therefore $S\in\lang{A'}$.

For the second direction, let $S\in\lang{A'}$. 
Then there exist $w_1,\ldots w_t\in S$, such that for every $w_{t+1},\ldots w_{k}$, it holds that $\hat\A'$ accepts $w' = \zip(w_1,\ldots w_k)$.
Then, by the conditions described above, $w'$ is a sequence of a word $w\in\lang{A}$ such that $\{w[1],\ldots w[t]\} = \{w'[1], \ldots w'[t]\} = \{w_1,\ldots w_t\}$ (though these words do not necessarily appear in the same order in $w,w'$), and such that $w[i] = w'[i]$ for every $t<i\leq k$. 
Then, by the semantics of the quantifiers, we have that $S\in\lang{\A}$.
\end{proof}

Notice that the $\nfhef$ $\A'$ of Lemma~\ref{lem:nfhef1} is permutation-sequence complete.

\begin{lemma}
Every $(k,t)-\nfhef$ $\A$ has an equivalent permutation-sequence complete $(k,t)-\nfhef$ $\A'$.
\end{lemma}
\begin{proof}
We construct $\A'$ in two steps. 
First, we construct $\A''$ that is the intersection of every $\A_\zeta$ for a sequence $\zeta$ of the form $(1,2,\ldots t, i_{t+1},\ldots i_k)$, as for $\nfhf$ over the last $k-t$ indices, and then we construct $\A'$ as the union of $\A''_\xi$ for every permutation $\xi$ of the form $(i_1,\ldots i_t,t+1,\ldots k)$, as for $\nfhe$ over the first $t$ indices.
\end{proof}

\begin{lemma}
Let $\A_1$ and $\A_2$ be two permutation-sequence complete $(k,t)-\nfhef$.
Then $\lang{\A_1}=\lang{\A_2}$ iff  $\lang{\hat\A_1} = \lang{\hat \A_2}$.
\end{lemma}
\begin{proof}
Suppose that $\lang{\A_1}=\lang{\A_2}$. Let $w\in\lang{\hat\A_1}$. 
Since $\A_1$ is permutation-sequence complete, we have that $w_\zeta\in\lang{\A_1}$ for every sequence $\zeta$ of the form $(1,\ldots t,i_{t+1},\ldots i_k)$. By the semantics of the quantifiers, we have that $\unzip{w}\in\lang{A_1}$.
Therefore, $\unzip{w}\in\lang{A_2}$, and so, according to the semantics of the quantifiers and the order of words in $w$, 
there exists a word $w'\in\lang{\hat\A_2}$ such that $(w'[1],\ldots w'[t])$ is a permutation of $(w[1],\ldots w[t])$, and $(w'[t+1],\ldots w'[k])$ is a permutation of $(w[t+1],\ldots w[k])$. Since $\A_2$ is permutation-sequence complete, we have that $w\in\lang{\hat\A_2}$. A similar argument shows that $\lang{\hat\A_2}\subseteq \lang{\hat\A_1}$.
The second direction is trivial.
\end{proof}

\begin{lemma}
Let $\A$ be a $(k,t)-\nfhef$, such that $k$ is the minimal number of variables needed for expressing $\lang{\A}$.
Then $\hat\A$ accepts a word $w$ in which $w[1],\ldots w[t]$ are all distinct. 
\end{lemma}
\begin{proof}
Suppose by way of contradiction that for every $w\in\lang{\hat\A}$, two of the first $t$ words of in $w$ are equal. Due to the semantics of the $\exists$ quantifier, we can also 
\end{proof}


\begin{lemma}
Let $\A_1$ and $\A_2$ be permutation-sequence complete $\nfhef$ for the same hyperlanguage $\cal L$, both with a minimal set of variables. Then the quantification conditions of $\A_1$ and $\A_2$ are equal.
\end{lemma}
\begin{proof}
Suppose that $\A_1$ is a $(t,k)-\nfhef$, and $\A_2$ is a $(t,m)-\nfhef$.
Suppose by way of contradiction, and without loss of generality, that $t < m$. 
Let $S\in\lang{\A_1}$. 
\end{proof}

We define a canonical form for $\nfhef$ as a minimal deterministic permutation-sequence complete $\nfhef$ with a minimal number of variables. 


}% of stam











==> hyper_regular.tex <==
\section{Hyperregular expressions}
\todo{Sarai: I think that we should drop the definition. We can say: We can represent a hyper-regular language $HL$ as a hyper-regular expression $\alpha r$, where $r$ is a regular expression for $\hat\A$ in an NFH $\A$ for $HL$, whose quantification condition is $\alpha$. I don't think we need more than that for this idea.}
A {\em hyper regular expression} (HRE) defines a hyperlanguage. HREs are 
inductively defined by the following grammar:
%
\todo{Sarai: there should also be $\emptyset$ in $\psi$, right?}
\begin{align*}
\varphi ::= & \ \forall x.\varphi \mid \exists x.\varphi \mid \psi\\
\psi ::= & \ \epsilon \mid (a_1, a_2, \ldots a_k) \mid \psi + \psi \mid 
\psi^* \mid \psi\psi
\end{align*}
% 
\todo{Sarai: since we use $k$-tuples, we should probably say that the set of HR is the set of closed (with $k$ quantifiers) expressions. Otherwise the semantics does not make sense.}
where $a_1, a_2, \dots, a_k$ are letters in a finite alphabet $\Sigma$ and $x$ 
is a word variable from an infinite supply $X$.

\todo{Sarai: the syntax and semantics should be separated. Regular expressions are the syntax. For every RE $r$, we assign a hyperlanguage $HL[r]$}The semantics of HREs is as follows. The following constants are 
defined as HREs (obtained by the $\psi$ rule): (1) the empty set $\emptyset$, 
(2) $\{\epsilon\}$ is an HRE, where $\epsilon$ is the empty word, and (3) a 
$k$-tuple of letters $(a_1, a_2, \ldots, a_k)$ is an HRE.
%
Furthermore, HREs can be obtained by the $\psi$ formulas as 
follows: 

\begin{itemize}
\item {\em Concatenation.} \ Let $R_1$ and $R_2$ be two sets of hyperwords. 
$R_1R_2$ denotes the set of hyperwords obtained by concatenating a hyperword in 
$R_1$ and a hyperword in $R_2$. We use the same padding technique for words 
with unequal lengths as described in Section~\ref{sec:ha}. Thus,
%
$$
R_1R_2 = \zip \Big(\unzip(R_1)\cdot\unzip(R_2)\Big)
$$
%
where `$\cdot$' denotes the the standard concatenation operator in regular 
expressions.
For example, let $R_1 
= \{(a, b, c)\}$, and $R_2 = \{(e_1, f_1)(\#, f_2)\}$. Then, 
$R_1R_2 = \{(a, a, b, b, c, c)(e_1, f_1, e_1, f_1)(\#, f_2, \#, 
f_2, \#, f_2)\}$.\todo{Sarai: I don't understand... why is this the concatenation?}

\item {\em Union.} \ $R_1 + R_2$ denotes the set union of sets described 
by $R_1$ and $R_2$:
%
$$
R_1 + R_2 = \zip\Big(\unzip(R_1) \, \cup \unzip(R_2)\Big)
$$
%
For example, if $R_1 = \{(a_1, b_1, a_2, b_2)\}$, and $R_2 
= \{(e_1, f_1)(e_2, f_2)\}$, expression $R_1 + R_2 = 
\{(a_1,b_1, a_2, b_2), (e_1, f_1 \#, \#)(e_2, f_2 \#, \#)\}$.

\item {\em Kleene star.} \ $R^*$ denotes the smallest superset of the set 
described by $R$ that contains $\epsilon$ and is closed under concatenation. 
This is the set of all hyperwords that can be made by concatenating any finite 
number (including zero) of hyperwords from the set described by $R$. For 
example, $((a, a) + (\bar{a}, \bar{a}))^*$, where $\bar{a} \in \Sigma - 
\{a\}$, is the hyperlanguage in which every pair of words agree on the 
position of letter $a$.

\end{itemize}
%
Finally, if $R$ is an HRE obtained by concatenation, alternation, and Kleen 
star only, then $\quant_1x_1.\quant_2x_2.\ldots 
\quant_nx_n R$, where $\quant_i \in \{\forall, \exists\}$, for all $i \in [1, 
n]$ is also an HRE. The semantics of quantified $\varphi$ formulas is the same 
as NHF described in Section~\ref{sec:haf}. 

\begin{theorem}

There is a direct one-to-one correspondence between the grammar of HRE and 
NHF, such that the grammar generates exactly the language the automaton accepts.

\end{theorem}

\begin{proof}
The construction is the same as the standard construction of an NFA from 
a regular expression. The quantification condition $\alpha$ of the NHF will be 
identical to the quantifiers of the input HRE. 
\end{proof}



% We clarify that an HRE cannot be obtained by (1) concatenating two quantified 
% expressions, and (2) applying Kleene star over a quantified expression. Also, 
% union should not created nested quantification.
%\subsection{Semantics of NFH}
% We now formally describe the semantics of NFH, and begin with some terms and 
% notations.


% The semantics of quantification is as follows. As we have noted, a hyperword 
% over $\Sigma$ is $S\subseteq \Sigma^*$. Let $X=\{x_1,\dots, x_k\}$ is a finite 
% set of {\em word variables} be a set of {\em word variables} and $v: 
% X\rightarrow S$ be an assignment of the word variables to words in $S$.
% We represent $v$ by the word $\zip(v) = \bi{v} = \zip(v(x_1),\ldots v(x_k))$.  
% 
% We now define the acceptance condition of a hyperword $S$ by an NFH $\A$. We 
% first define the satisfaction relation $\models$ for a hyperword $S$, an NFH 
% $\A$ over the set of variables $X = \{x_1,\ldots x_k\}$, a quantification 
% condition $\alpha$, and an assignment $v:X\rightarrow S$.
% 
% \begin{itemize}
%     \item For $\alpha = \epsilon$, we denote $S \models _v (\alpha,\A)$ iff 
% $\hat\A$ accepts $\zip(v)$. 
% 
% \item For $\alpha = \exists x_i \alpha'$, we denote $S\models_v \alpha,\A$ iff 
% there exists $w\in S$ such that $S \models_{v[x_i\rightarrow w]}  \alpha',\A$.
% 
% \item For $\alpha = \forall x_i \alpha'$, we denote $S\models_v \alpha',\A$ iff 
% for every $w\in S$, it holds that $S \models_{v[x_i\rightarrow w]}  \A$.
% 
% \end{itemize}
% When $\alpha$ includes all of $X$, then the satisfaction is independent of the 
% assignment $v$, and we denote $S \models \A$, in which case, we say that $\A$ 
% accepts $S$.





==> hyperbuchi.tex <==



==> learning_nfhef.tex <==
\subsection{Learning $\nfhef$}

We now describe a learning algorithm for $\nfhef$.
Our algorithm is based on Angluin's $L^*$ algorithm \cite{Angluin87} for regular languages, and aims to learn a minimal deterministic permutation-sequence complete $\nfhef$ with a minimal number of variables for a hyperlanguage $\cal L$.

As with $L^*$, our algorithm consists of two entities: a {\em learner} and a {\em teacher}.
During the learning process, the learner asks the teacher two types of queries: {\em membership queries} (``is the hyperword $S$ in $\cal L$?'') and {\em equivalence queries} (``Is $\A$ an $\nfhef$ for $\cal L$?'').


The number of variables, as well as the quantification condition $\alpha$, is unknown to the learner in advance, and is established during the learning procedure. 
In every step, the learner may cause one of the following to occur in the $\nfhef$ $\A$ that it maintains:
\begin{enumerate}
    \item Increase the number of states;
    \item Increase the number of variables;
    \item Turn an $\exists$ quantifier to a $\forall$ quantifier.
\end{enumerate}

As with $L^*$, the learner maintains an {\em observation table} $T$, which, intuitively, maintains the states and transitions of the underlying automaton that have been learned so far. In addition, the learner maintains the current number of variables $k$ (which also influences the alphabet of the observation table), and the number of $\exists$ quantifiers $t$ in the quantification condition. 

In case of a failed equivalence query, the teacher returns a {\em counterexample}: a {\em negative counterexample} is a hyperword that is not in $\lang{\A}$ and is in $\cal L$, and a {\em positive counterexample} is a hyperword that is in $\lang{\A}$, but is not in $\cal L$. We assume that the teacher always returns a minimal counterexample (in terms of set size).

The actions of the learner depend on the properties of the returned counterexample $S$ it gets from the teacher. 
We say that $S$ is {\em manifested} in $T$ if there exists a word $w$ in $T$ that is formed by zipping the words in $S$ in some order.
\begin{enumerate}
    \item 
    If $S$ is a positive counterexample of size $k$ or less, that is not manifested in $T$, then the learner adds  $\zip(S)$ to $T$, where $\zip(S)$ denotes zipping the words in $S$ in some arbitrary order. 
    \item 
    If $S$ is a positive counterexample of size $k$ or less, that is manifested in $T$, then the learner sets $t\leftarrow t-1$. 
    \item
    If $S$ is a positive counterexample of size $k'>k$, then the learner replaces every letter $\sigma$ in the transitions with $\uparrow^{k'}(\sigma)$, and sets $t\leftarrow t+(k'-k)$. 
    \item If $S$ is a negative counterexample, and $k>t$. then it must be that $S$ is of size $k$ or less, and does not already appear in $T$. The learner then adds $S$ to $T$.
    \item if $S$ is a negative counterexample of size $k'>k$, and $k=t$ (that is, the quantifiers are all $\exists$), then the learner sets $t\leftarrow t-1$.  
\end{enumerate}




\input{figures/learning_flow}



==> nfh_properties_full.tex <==
\section{Properties of Hyper Regular Languages}
\label{sec:nfh_properties}


In this section, we consider the basic operations and decision problems for the various fragments of NFH. 
Throughout  section, we assume an NFH $\A = \tuple{\Sigma,X,Q,Q_0,\delta,F,\alpha}$ where $X = \{x_1,\ldots x_n\}$. 

%For the various complexity results, notice that  the number of variables $k$ and the number of letters $\Sigma$ dictate an alphabet size of $O(|\Sigma|^k)$ for $\hat\A$. Thus, though the state space of $\hat\A$ is of size $n$, its size may be exponential in the number of variables due to its transition relation, which may be of size $n\times |\Sigma|^k\times n$. 


\begin{theorem} 
\label{thm:nfh.complement}

NFH are closed under complementation.

\end{theorem}


\begin{theorem} \label{thm:nfh.union}
NFH are closed under union.
\end{theorem}

\begin{theorem}\label{thm:nfh.intersection}


NFH are closed under intersection.
\end{theorem}


We now turn to study various decision problems for NFH. We begin with the 
nonemptiness problem: given an NFH $\A$, is $\hlang{\A} = \emptyset$? We show 
that while the problem is in general undecidable for NFH, it is decidable for 
most fragments that we consider. 


\begin{theorem}
\label{thrm:nonemptiness}

The nonemptiness problem for NHF is undecidable.
\end{theorem}



\begin{theorem} \label{thm:nfhe.nfhf.nonemptiness}
The nonemptiness problem for $\nfhe$ and $\nfhf$ is \comp{NL-complete}.
\end{theorem}

We now show that the nonemptiness problem for $\nfhef$ is decidable. We first 
present some terms and notations.  

Consider a tuple $t = (t_1,t_2,\ldots t_k)$ of items. 
A {\em sequence} of $t$ is a tuple $(t'_1, t'_2,\ldots t'_k)$, where 
$t'_i\in\{t_1,\ldots t_k\}$ for every $1\leq i \leq k$. 
A {\em permutation} of $t$ is a reordering of the elements of $t$. 
We extend the notion of permutation to words over $k$-tuples, and to 
assignments, as follows. 
Let $w = \zip(w_1,\ldots w_k)$ be a word over $k$-tuples, and let $\zeta = 
(i_1,i_2,\ldots i_k)$ be a sequence (permutation) of $(1,2,\ldots, k)$. The word $w_\zeta$, 
defined as $\zip(w_{i_1}, w_{i_2}, \ldots w_{i_k})$ is a sequence (permutation) of $w$.
Finally, let $v$ be an assignment from a set of variables $\{x_1,x_2,\ldots 
x_k\}$ to a hyperword $S$. The assignment $v_\zeta$, defined as $v_\zeta(x_j) = 
v(x_{i_j})$ for every $1\leq i,j \leq k$, is a sequence (permutation) of $v$. 
\todo{Sarai: move this elsewhere? since we use these terms also in learning}

We now show that if an $\nfhef$ is nonempty, then we can bound the size of a 
hyperword that it accepts.

\begin{lemma}\label{lemma:nfhef.nonempty}
Let $\A$ be an $\nfhef$ with a quantification condition $\alpha = \exists x_1,\ldots \exists x_m \forall 
x_{m+1}\ldots \forall x_k$, where $1 \leq m < k$. 
Then $\A$ is nonempty iff $\A$ accepts a hyperword of size at most $m$.
\end{lemma}


We now use Lemma~\ref{lemma:nfhef.nonempty} to describe a decision procedure for 
the nonemptiness of $\nfhef$. 

\begin{theorem}\label{thm:nfhef.nonemptiness}
The nonemptiness problem for an $\nfhef$ $\A$ can be decided in space that is 
polynomial in the size of $\hat\A$.
\end{theorem}


\begin{theorem}
\label{thrm:nonemptinessEA}
The nonemptiness problem for $\nfhef$ is  \comp{PSPACE-complete}.
\end{theorem}

We turn to study the membership problem for NFH: given an NFH $\A$ and a 
hyperword $S$, is $S\in\hlang{\A}$? 
When $S$ is finite, the set of assignments from $X$ to $S$ is finite, and so the problem is decidable. We call this case the {\em finite membership problem}. 

\begin{theorem}\label{thm:nfh.membership.finite}
Let $\A$ be an NFH and $S$ be a finite hyperword over $\Sigma$. Then it can be 
decided whether $S\in \hlang{\A}$ in space that is polynomial in $k$, and 
logarithmic in $|\hat\A|, |S|$.
\end{theorem}

\begin{proof}
As discussed in the proof of Theorem~\ref{thm:nfhef.nonemptiness}, the size of 
$\hat\Sigma$ must be exponential in the number of $\forall$ quantifiers in 
$\alpha$, and therefore is exponential in $k$. We can decide the membership of 
$S$ in $\hlang{\A}$ by iterating over all assignments of the type $X\rightarrow 
S$. For every such assignment $v$, we construct $\zip(v)$ and run $\hat\A$ on 
$\zip(v)$, on-the-fly. 
\end{proof}

The exponential size of $\hat\A$ is derived from the number of $\forall$ 
quantifiers. When the number of $\forall$ quantifiers is fixed, then 
$\hat\Sigma$ is not necessarily exponential in $k$. 

\begin{theorem}
\label{thrm:membershipA}
The finite membership problem for NFH with a fixed number of $\forall$ 
quantifiers is \comp{NP-complete}.
\end{theorem}

When $S$ is infinite, it may still be finitely represented. 
We now address the problem of deciding whether a regular language $\cal L$ 
(given as an NFA) is accepted by an NFH. We call this {\em the regular 
membership problem for NFH}. We show that this problem is decidable for the 
entire class of NFH. 

\begin{theorem}
\label{thrm:membershipFULL}
The regular membership problem for NFH is decidable.
\end{theorem}


\begin{theorem}
\label{thrm:inclusion}
 The inclusion problems of $\nfhe$ and $\nfhf$ in $\nfhe$ and $\nfhf$ and of 
$\nfhef$ in $\nfhe$ and $\nfhf$ are \comp{PSPACE-complete}.
\end{theorem}

\iffalse

\subsection{Properties of NBH}

Since NBWs are closed under the Boolean operations, and their nonemptiness and inclusion problems are decidable (and are NL-complete and PSPACE-complete, respectively), the results of Section~\ref{sec:nfh_properties} can all be lifted to the case of hyper-infinite words. 
To summarize, we have the following. 

\begin{theorem}
\begin{itemize}
    \item NBH are closed under the Boolean operations.
    \item The nonemptiness problem for NBH$_\exists$ is NL-complete.
    \item The nonemptiness problem for NBH$_{\exists\forall}$ is decidable in EXPSPACE.
    \item The nonemptiness problem for NFH$_{\forall\exists}$ is undecidable.
    \item The $\omega$-regular membership problem for NBH is decidable.\todo{this is just a bit trickier, since we need to be more careful with the accepting states}
\end{itemize}
\end{theorem}

\fi

==> nfhef_nonemptiness.tex <==
\begin{theorem}
The nonemptiness problem for $\nfhef$ is EXPSPACE-complete w.r.t. $n,k$ and PSPACE-complete w.r.t. $|\hat A|$.
\end{theorem}
\begin{proof}
The upper bound follows from Theorem~\ref{thm:nfhef.nonemptiness}. 
For the lower bound, we show a reduction from an exponent version of the {\em tiling problem}~\cite{Boas97}, defined as follows.
We are given a finite set $T$ of tiles, two relations $V \subseteq T \times T$ and $H \subseteq T \times T$,
an initial tile $t_0$, a final tile $t_f$, and a bound $n>0$.
We have to decide whether there is some $m>0$ and a tiling of a $2^n \times m$-grid such that
(1) The tile $t_0$ is in the bottom left corner and the tile $t_f$ is in the top left corner,
(2) A horizontal condition: every pair of horizontal neighbors is in $H$, and
(3) A vertical condition: every pair of vertical neighbors is in $V$.
Formally, we have to decide whether there exist $m\in \N$ and a function $f:\{0,\ldots,2^n-1\} \times \{0,\ldots,m-1\} \rightarrow T$
such that
(1) $f(0,0)=t_0$ and $f(0, m-1)=t_f$,
(2) For every $0 \leq i \leq 2^n-2$ and $0 \leq j \leq m-1$, we have that $(f(i,j),f(i+1,j)) \in H$, and
(3) For every $0 \leq i \leq 2^n-1$ and $0 \leq j \leq m-2$, we have that $(f(i,j),f(i,j+1)) \in V$.
When $n$ is given in unary, the problem is known to be EXPSPACE-complete.

Given an instance $C$ of the tiling problem, We construct an $\nfhef$ $\A$ that is nonempty iff $C$ has a solution. 
We encode a solution to $C$ as a word $w_{sol} =w_1\cdot w_2\cdot w_m\$$ over $T$, where $w_i$, of the form $t_{1,i}t_{2,i},\ldots t_{2^n,i}$, describes the contents of row $i$. 

To make sure that $w_{sol}$ is indeed a solution, we need to make sure that:
\begin{enumerate}
\item $w_1$ begins with $t_0$ and $w_m$ ends with $t_f\$$,
\item Within every $w_i$, it holds that $(t_{j,i},t_{j+1,i})\in H$,
    \item Every row is of length $2^m$,
    \item For $w_i,w_{i+1}$, it holds that $(t_{j,i}, t_{j,i+1})\in V$ for every $1\leq j\leq 2^n$
\end{enumerate} 

Verifying items $(1-2)$ is easy via an NFA.  
The main obstacles are items $(3-4)$. 

To make sure that the rows are of length $2^n$, we encode the horizontal positions using $n$ bits. The bits are described by a set of letters $B = \{b_{1,0}, b_{1,1},\ldots b_{n,0},b_{n,1}\}$, where $b_{k,v}$ means that the value of the $k$'th bit is $v$. 

We extend the representation of a solution $w_sol$ to $n$ different words $w_{sol,1},\ldots w_{sol, n}$, where the $w_{sol,k}$ denotes the word obtained from $w_{sol}$ by adding, before each letter $t_{j,i}$, the letter $b_{k,v}$, where $v$ is the value of the $k$'th bit in the encoding of $j$. 

Thus, a solution to $C$ is now $W = \zip(w_{sol,1},\ldots w_{sol,n})$.
For example, for $k=3$, the first two letters of $W$ are of the form $$(b_{1,0},b_{2,0},b_{3,0}),(t_{1,1}, t_{1,1},t_{1,1}),(b_{1,0},b_{2,0},b_{3,1}),(t_{2,1},t_{2,1},t_{2,1})$$.

We describe an $\nfhef$ $\A_1 = \tuple{T\cup B, \{x_1,\ldots x_{2n}\}, Q, \{q_0\},\delta, F, \alpha}$ that is nonempty iff there exists a word that satisfies items $(1-3)$.
The quantification condition $\alpha$ is $\exists x_1\ldots \exists x_n \forall y_1 \ldots \forall y_n$.

$\A_1$ only proceeds on letters in $B^{2n}$ (bit letters) or of the form $t^{2n}$ (or $(t_f\&)^{2n})$, for $t\in T$ (tile letters). 
Further, it makes sure of the following.
\begin{enumerate}
    \item $W$ alternates between bit letters and tile letters. 
    \item The first $n$ positions of the first letter are of the form $b_{1,v},b_{2,v},\ldots b_{n,v}$.
    \item For every $W[i]$, there only appear bits from the same position. That is, $W[i]$ does not contain both $b_{j,v}, b_{j',v'}$ for $j\neq j'$.
    \item The conditions for $t_0, t_f$, and $H$ are all met.
\end{enumerate}

All these conditions can be checked separately for either each letter or each word $W[i]$. 

Correct enumeration is checked as follows. 
There exists some $k$ for which $W[n+1]$ contains only $B$ letters for position $k$. 
Depending on the value of $k$, the states in $\A$ make sure that the bit values conform to the $k$'th bit in a counter. For example, if $n=4$, then for $k=4$ the sequence of values should be $(0,1,0,1,\ldots)$, and for $k=3$ the sequence should be $(0,0,1,1,0,0,1,1,\ldots)$.

It suffices to check every bit separately, since the $\forall$ requirement is that every representation of a word $W$ should be accepted, and so every position $k$ should appear in $W[n+1]$ in some representation of $W$. Therefore, $W$ can be accepted iff every bit conforms to its behaviour in a $2^n$ counter. 

We proceed to describe how to extend $\A_1$ to handle the requirement for $V$. 
We need to make sure that for every position $j$ in a row, the tile in position $j$ in the next row matches the current one. Since he number of positions is exponential in $n$, we cannot use the states to remember $j$.
Instead, we add words that determine the position $j$ that is to be remembered. 
We add to the alphabet a set of new bit letters $C = \{c_{1,0},c_{1,1},c_{2,0},c_{2,1},\ldots c_{n,0}, c_{n,1}\}$. 
Intuitively, words over $C$ will contain exactly one bit letter $c_{i,v}$ each. A set of $n$ such words, one for each $1\leq i\leq n$, determines the position that is to be checked. 
The extended $\nfhef$ $\A$ requires the existence of these $2n$ constant words under $\exists$ quantifiers, and for words in $\hat\A$ that contain $n$ appropriate words under the $\forall$ quantifiers, $\A$ requires that in every two consecutive positions that conform to the position encoded by these words, the two matching tiles are in $V$. 

Accordingly, $\alpha$ is extended to $\exists x_1\ldots \exists x_n \exists v_1 \ldots \exists v_{2n} \forall y_1\ldots \forall y_n \forall v_1\ldots \forall v_n$, and $\hat\A$ reads letters of the type $t^{5n}$ or of the type $B^n\cdot C^{2n} \cdot (B\cup C)^{2n}$. 
The following requirements are added to the requirements listed above for $\A_1$:
\begin{enumerate}
    \item positions $n+1$ to $3n$ are  $c_{1,0},\ldots c_{n,0}, c_{1,1},\ldots c_{n,1}$.
    \item If a word $W[i]$ starts with some $c_{i,v}$, then $c_{i,v}$ occurs in all odd positions in $W[i]$ (recall that the even positions are tiles). 
    \item Every word in which positions $3n+1$ to $4n$ does not start with a letter in $B$, or positions $4n+1$ to $5n$ does not start with a letter in $C$, such that every $1\leq i \leq n$ is represented in $C$, is accepted. 
\end{enumerate}

Now, consider a word in which positions $3n+1$ to $4n$ start with letters in $B$ representing every position $1$ to $n$, and positions $4n+1$ to $5n$ start with letters in $C$, also representing every such position. 
The $C$ values determine the position within the rows that should be checked. Whenever the $C$ values match the $B$ values, $\A$ uses the states to remember the tile $t$ in the next letter, and the next time that the $C$ and $B$ values are matched, it checks that the following tile $t'$ satisfies $(t,t')\in V$ (and remembers $t'$ for the next check).
Since every sequence must be accepted, we have that for a hyperword to be accepted, every row position must be tested in some assignment, and so the solution must also satisfy $V$.

\end{proof}


==> theorem12.tex <==
\begin{theorem}
Let $k'$ be the number of variables under $\forall$.
\begin{itemize}
    \item If $k'= O(\log(k))$ then the membership problem is NP-complete.
    \item
    If $k = O(k')$ then the membership problem is NL-complete.
\end{itemize}

\end{theorem}

\begin{proof}
Let $S$ be a hyperword of size at least $2$, and let $\A$ be an NFH. 

We can solve the membership problem for $\A$ and $S$ by iterating over relevant assignments from $X$ to $S$, and for every such assignment $v$, checking whether $\zip(v)$ is accepted by $\hat\A$. 
This algorithm uses space of size that is polynomial in $k$ and logarithmic in $|\A|$ and in $|S|$. 

To account for all the assignments to the $\forall$ variables, $\delta$ -- and therefore, $\hat\A$ -- must be of size at least $2^{k'}$ (otherwise, we can return ``no'').
We then have that if $k = O(k')$, then space of size $k$ is logarithmic in $|\hat\A|$, and so the problem in this case can be solved within logarithmic space.
The lower bound follows from the membership problem for NFA. 

In the case that $k' = O(\log k)$, iterating over 
all assignments to the variables under $\forall$, while guessing assignments to 
the variables under $\exists$ is done in polynomial time. For each such assignment $v$, checking whether $\zip(v)\in\lang{\hat\A}$ can be done on-the-fly. 
Notice that now we cannot claim that the size of $\delta$ is exponential in 
$k$. Therefore, the described solution provides membership in 
\comp{NP}. 

We show \comp{NP-hardness} for this case by a reduction from the Hamiltonian cycle problem. 
Given a graph $G = \tuple{V,E}$ where $V = \{v_1,v_2,\ldots v_n\}$ and $|E|=m$, 
we construct an $\nfhe$ $\A$ over $\{0,1\}$ with $n$ states, $n$ variables, 
$\delta$ of size $m$, and a hyperword $S$ of size $n$, as follows. $S = 
\{w_1,\ldots w_n\}$, where $w_i$ is the word over $\{0,1\}$ in which all letters 
are $0$ except for the $i$'th. 
The structure of $\hat\A$ is identical to that of $G$, and we set $Q_0 = F = 
\{v_1\}$. For the transition relation, for every $(v_i,v_j)\in E$, we have 
$(v_i, \sigma_i,v_j)\in \delta$, where $\sigma_i$ is the letter over $\{0,1\}^n$ 
in which all positions are $0$ except for position $i$. 
Intuitively, the $i$'th letter in an accepting run of $\hat\A$ marks traversing 
$v_i$. Assigning $w_j$ to $x_i$ means that the $j$'th step of the run 
traverses $v_i$. Since the words in $w$ make sure that every $v\in V$ is 
traversed exactly once, and that the run on them is of length $n$, we have that 
$\A$ accepts $S$ iff there exists some permutation $p$ of the words in $S$ such 
that $p$ matches a Hamiltonian cycle in $G$.
\end{proof}
